SLAMP: Stochastic Latent Appearance and Motion Prediction

Motion is an important cue for video prediction and often utilized by separating video content into static and dynamic components. Most of the previous work utilizing motion is deterministic but there are stochastic methods that can model the inherent uncertainty of the future. Existing stochastic models either do not reason about motion explicitly or make limiting assumptions about the static part. In this paper, we reason about appearance and motion in the video stochastically by predicting the future based on the motion history. Explicit reasoning about motion without history already reaches the performance of current stochastic models. The motion history further improves the results by allowing to predict consistent dynamics several frames into the future. Our model performs comparably to the state-of-the-art models on the generic video prediction datasets, however, significantly outperforms them on two challenging real-world autonomous driving datasets with complex motion and dynamic background.

==> sec/var_inf_temp.tex <==
For the generation of the future frames, the conditional joint probability of our model with only motion can be written as,

\begin{align}
    p(\bx_{1:T}) = \prod_{t=1}^{T} p(\bx_t | \bg_t)\  p(\bg_t | \bz_t, \bx_{t-1})\  p(\bz_t)
\end{align}

\begin{align}
    p(\bx_{1:T}) = \prod_{t=1}^{T} p(\bx_t | \bz_t, \bx_{t-1})\  p(\bz_t | \bz_{t-1}, \bx_{1:t-1})
\end{align}

\ka{ilk denklemde $g_t$ introduce ettim ama gerek olmayabilir diye digerini de yazdim, tam olarak emin degilim.}

In order to optimize the likelihood of $p(\bx_{1:T})$, we need to infer latent variable, $\bz_t$, which corresponds to uncertainty in the future frames. We used variational inference model, parameterized by $\bphi$, to infer latent variables. The variational distribution is,

\begin{align}
    q_{\bz} = \prod_{t=1}^{T} q_{\bphi}(\bz_t | \bx_{1:T})
\end{align}

Since the $\bz_1, ..., \bz_T$ are independent across time, we can further decompose Kullback-Leibler term to optimize latent distributions into individual time steps. Evidence lower bound (ELBO) is as follows:

\ka{ELBO SVG ile ayni oluyor sanirsam motion olmayan case'de, ya da $p_{\btheta}$'yi introduce ederken 2 farkli yerden alip fuse ettigimizi mi soylemek gerekiyor bilemedim.}

\begin{align*}
    \mathrm{log}\ p_{\btheta}(\bx) &\geq L_{\btheta,\bphi}(\bx_{1:T}) \\
        &= \mathbbm{E}_{q_{\phi}(\bz | \bx)} \mathrm{log}\ p_{\btheta}(\bx_t | \bx_{1:t-1}, \bz_{1:t}) \\
        &= \sum\limits_{t} [\mathbbm{E}_{q_{\phi}(\bz_{1:t} | \bx_{1:t})}\mathrm{log}\ p_{\btheta}(\bx_t | \bx_{1:t-1}, \bz_{1:t}) \\
        &\quad \quad - \KLD{q_{\bphi}(\bz_t | \bx_{1:t})}{p_{\bpsi}(\bz_t|\bx_{1:t-1})}]
\end{align*}


We are training the model with Motion by optimizing the variational lower bound. The likelihood term in the equation, $p_{\btheta}$, can be interpreted as an $l_2$ penalty between $\bx_t$ and $\hat{\bx_t}$. The posterior and prior terms are estimated as an expectation over $q_{\bphi}(\bz_{1:t} | \bx_{1:t})$ and $p_{\bpsi}(\bz_t|\bx_{1:t-1})$, respectively. We used re-parameterization trick used in \cite{Kingma2014ICLR}.

\textbf{ELBO FOR MODEL WITH MOTION HISTORY}
%
\begin{align*}
    p(\bx_{1:T}) &= \prod_{t=1}^{T}  p(\bx_t \lvert \bz_t^p, \bz_t^f, \bx_{t-1}, \bx_{t-2}) \\
    & p(\bz_{t}^{p} \lvert \bz_{t-1}^{p}, \bx_{1:t-1})  p(\bz_{t}^{f} \lvert \bz_{t-1}^{f}, \bx_{1:t-1})
\end{align*}
%
\ka{burada belki ilk kisim icin, $\bx_{t-1}, \bx_{t-2}$ yerine $\bx_{1:t}$ yazilabilir. }


We used a variational inference model, parameterized by $\bphi^{p}$ and $\bphi^{f}$, to infer latent variables. The variational distribution is,
%
\begin{align}
    q_{\bz}^{p} &= \prod_{t=1}^{T} q_{\bphi}^{p}(\bz_{t}^{p} | \bx_{1:T}) \\
    q_{\bz}^{f} &= \prod_{t=1}^{T} q_{\bphi}^{f}(\bz_{t}^{f} | \bx_{1:T}) \\
\end{align}

\ka{ELBO ikinci siradaki denklem icin, expectation'i 2 independent distribution uzerinden hesaplarsak o sekilde yazabiliyoruz. Posteriorlar hesaplanis bicimi olarak birbirlerinden bagimsiz duruyor ama ikisinde de target frame'e bir dokunus var (t=1 icin $x_2$). biraz daha dikkatli incelemek gerekebilir. }

% \begin{align*}
%     \bmu_{\bphi(t)}, \bsigma_{\bphi(t)} &= \mathrm{LSTM}_{\bphi}(\bh_t) &&& \bh_t = \mathrm{Enc}(\bx_t) \\
%     \bz_t &\sim \mathcal{N}(\bmu_{\bphi(t)}, \bsigma_{\bphi(t)}) \\
%     \bmu_{\bpsi(t)}, \bsigma_{\bpsi(t)} &= \mathrm{LSTM}_{\bpsi}(\bh_{t-1}) &&& \bh_{t-1} = \mathrm{Enc}(\bx_{t-1}) \\
%     \bz_t &\sim \mathcal{N}(\bmu_{\bpsi(t)}, \bsigma_{\bpsi(t)}) \\
%     \bg_t &= \mathrm{LSTM}_{\btheta}(\bh_{t-1}, \bz_t)  &&& \bh_{t-1} = \mathrm{Enc}(\bx_{t-1}) \\
%     \bmu_{\btheta}^{pix} &= \mathrm{PixDec}(\bg_t) \\
%     \bmu_{\btheta}^{flow} &= \mathrm{FlowDec}(\bg_t) \\
%     \bmu_{\btheta}^{mask} &= \mathrm{MaskDec}(\bg_t)
% \end{align*}


% \begin{align*}
%     \begin{split}
%          \mathrm{log}\ p_{\btheta}(\bx) &\geq L_{\btheta,\bphi^{p}, \bphi^{f}}(\bx_{1:T})
%     \end{split} \\
%     \begin{split}
%         = &\mathbbm{E}_{\substack{q_{\phi}^{p}(\bz^{p} \lvert \bx) \\ 
%                                   q_{\phi}^{f}(\bz^{f} \lvert \bx)}}
%         ~~\mathrm{log}\ p_{\btheta}(\bx \lvert \bz^p, \bz^f) \\
%          - &\KLD{q^p_{\phi}(\bz^p \lvert \bx)}{p^p_{\psi}(\bz^p)} \\
%          - &\KLD{q^f_{\phi}(\bz^f \lvert \bx)}{p^f_{\psi}(\bz^f)}
%     \end{split} \\
%     \begin{split}
%         = \mathbbm{E}_{\substack{q_{\phi}^{p}(\bz^{p} \lvert \bx) \\ 
%                                   q_{\phi}^{f}(\bz^{f} \lvert \bx)}}
%         ~~\mathrm{log}\ p_{\btheta}(\bx \lvert \bz^p, \bz^f) \\
%         - \KLD{q^p_{\phi}(\bz^p \lvert \bx)}{p^p_{\psi}(\bz^p)} \\
%         - \KLD{q^f_{\phi}(\bz^f \lvert \bx)}{p^f_{\psi}(\bz^f)} 
%     \end{split}\\
%     \begin{split}
%         = \sum\limits_{t}
%             \mathbbm{E}_{\substack{q_{\phi}^{p}(\bz_{1:t}^{p} \lvert \bx_{1:t}) \\                                           q_{\phi}^{f}(\bz_{1:t}^{f} \lvert \bx_{1:t})}}
%         ~~\mathrm{log}\ p_{\btheta}(\bx_t \lvert \bx_{1:t-1}, \bz_{1:t}^{p}, \bz_{1:t}^{f}) \\
%         - \KLD{q_{\bphi}^{p}(\bz_{t}^{p} \lvert \bx_{1:t})} {p_{\bpsi}^{p}(\bz_{t}^{p} \lvert \bx_{1:t-1})} \\ 
%         - \KLD{q_{\bphi}^{f}(\bz_{t}^{f} \lvert \bx_{1:t})} {p_{\bpsi}^{f}(\bz_{t}^{f} \lvert \bx_{1:t-1})}
%     \end{split}
% \end{align*}


    % &= \begin{aligned}[t]
    %     %  \mathbbm{E}_{\substack{q_{\phi}^{p}(\bz^{p} \lvert \bx) \\ 
    %     %                          q_{\phi}^{f}(\bz^{f} \lvert \bx)}}
    %      \mathbbm{E}_{ q_{\phi}^{\boldsymbol{\cdot}}(\bz^{\cdot} \lvert \bx)}
    %      &~\mathrm{log}\ p_{\btheta}(\bx \lvert \bz^p, \bz^f) \nonumber \\
    %      &- \KLD{q^{\cdot}_{\phi}(\bz^{\cdot} \lvert \bx)}{p^{\cdot}_{\psi}(\bz^{\cdot})} \\
    %      %&- \KLD{q^f_{\phi}(\bz^f \lvert \bx)}{p^f_{\psi}(\bz^f)}
    % \end{aligned}\\
    % &={} \begin{aligned}[t]
    %     % \mathbbm{E}_{\substack{q_{\phi}^{p}(\bz^{p} \lvert \bx) \\ 
    %     %                         q_{\phi}^{f}(\bz^{f} \lvert \bx)}}
    %     \mathbbm{E}_{q_{\phi}^{\cdot}(\bz^{\cdot} \lvert \bx)}
    %     &~\mathrm{log}\ p_{\btheta}(\bx \lvert \bz^p, \bz^f) \nonumber \\
    %     &- \KLD{q^{\cdot}_{\phi}(\bz^{\cdot} \lvert \bx)}{p^{\cdot}_{\psi}(\bz^{\cdot})} \\
    %     %&- \KLD{q^f_{\phi}(\bz^f \lvert \bx)}{p^f_{\psi}(\bz^f)} 
    % \end{aligned}\\
    % &={} \begin{aligned}[t]
    %     \sum\limits_{t}
    %         % \mathbbm{E}_{\substack{q_{\phi}^{p}(\bz_{1:t}^{p} \lvert \bx_{1:t}) \\                                           q_{\phi}^{f}(\bz_{1:t}^{f} \lvert \bx_{1:t})}}
    %         \mathbbm{E}_{q_{\phi}^{\cdot}(\bz_{1:t}^{\cdot} \lvert \bx_{1:t})}
    %     &~\mathrm{log}\ p_{\btheta}(\bx_t \lvert \bx_{1:t-1}, \bz_{1:t}^{p}, \bz_{1:t}^{f}) \\
    %     &- \KLD{q_{\bphi}^{\cdot}(\bz_{t}^{\cdot} \lvert \bx_{1:t})} {p_{\bpsi}^{\cdot}(\bz_{t}^{\cdot} \lvert \bx_{1:t-1})} \nonumber \\ 
    %     %&- \KLD{q_{\bphi}^{f}(\bz_{t}^{f} \lvert \bx_{1:t})} {p_{\bpsi}^{f}(\bz_{t}^{f} \lvert \bx_{1:t-1})}
    % \end{aligned}\\

==> tab/fvd.tex <==
\begin{table*}[h!]
    \captionsetup[table]{justification=centering}
    \sisetup{detect-weight, table-align-uncertainty=true, mode=text}
    \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
    \renewrobustcmd{\boldmath}{}
    \caption{
        \label{tab:fvd}
        \textbf{FVD Scores on the KTH and BAIR.} This table compares all the methods in terms of FVD scores with their $95\%$-confidence intervals over five different samples from the models. Our model is the second best on KTH and among top three methods on BAIR.}
    \centering
    \vspace{-0.05in}
    \small
    \begin{tabular}{lS[table-format=3(2)]S[table-format=3(2)]S[table-format=3(2)]S[table-format=3(2)]S[table-format=3(2)]S[table-format=3(2)]S[table-format=3(2)]S[table-format=3(2)]}
        \toprule
        Dataset & {SV2P} & {SAVP} & {SVG} & {SRVP} & {SLAMP - Baseline} & {SLAMP} \tabularnewline
        \midrule
        KTH & 636 $\pm$ 1 & 374 $\pm$ 3 & 377 $\pm$ 6 & \bfseries 222 $\pm$ 3 & 236 $\pm$ 2 & \underline{228} $\pm$ 5 \tabularnewline
        BAIR & 965 $\pm$ 17 & \bfseries 152 $\pm$ 9 & 255 $\pm$ 4 & \underline{163} $\pm$ 4 & 245 $\pm$ 5 & {\textemdash} \tabularnewline
        \bottomrule
    \end{tabular}
    \vspace{-2mm}
\end{table*}

